Detecting Shadow AI: Unsanctioned LLM Agents on Enterprise Endpoints: A Taxonomy, an Open Detector and a Controlled Evaluation

Shadow IT, the use of technology that the IT organisation has not approved, is a long-standing governance problem. We argue that autonomous AI agents can make it grow much faster: agents make building tools nearly free, act with their user's privileges, and leave behind scripts, automations and MCP servers that are themselves unsanctioned. A simple compounding model shows that, under its assumptions, shadow IT grows exponentially once agentic artifacts reproduce faster than the organisation retires them; retiring them starts with detecting them. We then ask whether unsanctioned agents can be detected on Windows endpoints. We propose a taxonomy of nine classes of agents and six layers of endpoint footprint, and argue that rules based only on the structure of processes and connections cannot separate an agent from its behavioural twin, the same program talking to a non-AI service. We present Agent Detector, an open-source Windows detector that anchors behaviour to the identity of the remote service and correlates it with configuration, installation and execution history, using a catalog of 39 tools and 184 LLM endpoint entries; it informs users through a notice they must acknowledge instead of blocking. On a controlled bench of 12 synthetic agents, 3 AI components and 9 benign workloads, repeated 5 times on one workstation, two behavioural rules flagged every behavioural twin, while Agent Detector flagged none and detected every agent in the majority of runs. Its limits are temporal: a connection to a provider behind a shared content-delivery network is attributable only while the DNS cache holds the provider's name, one to five minutes, and an intermittent agent was seen by about one scan in three. A scan costs about 154 ms. The bench is too small to rank detectors; it maps what each kind of evidence can see: unsanctioned agents can be partly detected, and not by behaviour alone.

==> eval/results/tex/tab-episodes-admin.tex <==
\begin{tabular}{@{}l >{\raggedright\arraybackslash}p{2.4cm} >{\raggedright\arraybackslash}p{4.4cm} c c c c >{\raggedright\arraybackslash}p{3.0cm}@{}}
\toprule
Id & Class & Episode & D0 & D1 & D2 & AD & Agent Detector findings \\
\midrule
A01 & Model provider (CDN-hosted) & Python agent, OpenAI API, persistent cmd & \xmark & \cmark & \cmark & \cmark & probable-agent \\
A02 & Model provider (dedicated range) & Python agent, Anthropic API, persistent cmd & \xmark & \cmark & \cmark & \cmark & llm-api, probable-agent \\
A03 & Model provider (dedicated range) & Node.js agent, Anthropic API, persistent PowerShell & \xmark & \cmark & \cmark & \cmark & llm-api, probable-agent \\
A04 & Model provider (CDN-hosted) & PowerShell agent, Mistral API, persistent cmd & \xmark & \cmark & \cmark & \cmark & probable-agent \\
A05 & Aggregator & Python agent, OpenRouter, persistent cmd & \xmark & \cmark & \cmark & \cmark & probable-agent \\
A06 & Inference platform & Python agent, Groq API, persistent cmd & \xmark & \cmark & \cmark & \cmark & probable-agent \\
A07 & Unknown relay (declared) & Python agent through a relay set in OPENAI\_BASE\_URL & \xmark & \cmark & \cmark & \cmark & probable-agent, relay-candidate \\
A08 & Local LLM & Local LLM-style server on port 11434 and an agent using it & \xmark & \xmark & \xmark & \cmark & local-llm-server, probable-agent \\
A09 & Agent with MCP server & Python agent, Anthropic API, reference MCP filesystem server & \xmark & \cmark & \cmark & \cmark & llm-api, probable-agent \\
A10 & Agent driving a browser & Python agent, Anthropic API, headless Chrome with remote debugging, no shell & \xmark & \xmark & \xmark & \cmark & llm-api \\
A11 & Renamed runtime & Node.js agent run by a copy of node.exe renamed updater.exe & \xmark & \xmark & \cmark & \cmark & llm-api, probable-agent \\
A12 & Intermittent agent & Python agent, Anthropic API, a call every 10 s, connection closed after 5 s, one short shell per call & \xmark & \cmark & \cmark & \xmark & -- \\
\midrule
C01 & Inference runtime & Process loading a module named like an inference runtime (ggml), no network & \xmark & \xmark & \xmark & \cmark & local-llm-runtime \\
C02 & MCP server & Reference MCP filesystem server alone, no LLM connection & \xmark & \cmark & \cmark & \cmark & mcp-server \\
C03 & LLM client without tools & Python script polling the Anthropic API, no shell, no tools & \xmark & \xmark & \xmark & \cmark & llm-api \\
\midrule
B01 & Behavioural twin & Twin of A02: Python script, PyPI JSON API, persistent cmd & \xmark & \cmark & \cmark & \xmark & -- \\
B02 & Behavioural twin & Twin of A03: Node.js script, npm registry, persistent PowerShell & \xmark & \cmark & \cmark & \xmark & -- \\
B03 & Behavioural twin & Twin of A04: PowerShell script, Microsoft Graph, persistent cmd & \xmark & \cmark & \cmark & \xmark & -- \\
B04 & Developer workload & npm install with install script (cmd) & \xmark & {\scriptsize 4/5} & {\scriptsize 4/5} & \xmark & -- \\
B05 & Developer workload & git clone over HTTPS & \xmark & \xmark & \xmark & \xmark & -- \\
B06 & Developer workload & pip download of a large wheel & \xmark & \xmark & \xmark & \xmark & -- \\
B07 & Developer workload & dotnet restore and build & \xmark & \xmark & \xmark & \xmark & -- \\
B08 & Developer workload & go build with module download & \xmark & \xmark & \xmark & \xmark & -- \\
B09 & Inherited base URL & git loop in a PowerShell that inherited OPENAI\_BASE\_URL from the user environment & \xmark & \xmark & \xmark & \xmark & -- \\
\midrule
R01 & Undeclared relay & Python agent through a relay hard-coded in the script & \xmark & \cmark & \cmark & \xmark & -- \\
R02 & Ephemeral agent & Python agent running 5 s, scanned after it exited & \xmark & \xmark & \xmark & \xmark & -- \\
R03 & Agent inside WSL 2 & Python agent running in the Ubuntu WSL 2 distribution & \xmark & \xmark & \xmark & \xmark & -- \\
\bottomrule
\end{tabular}


==> eval/results/tex/tab-insitu-admin.tex <==
\begin{tabular}{@{}>{\raggedright\arraybackslash}p{3.2cm} >{\raggedright\arraybackslash}p{5.4cm} l l c@{}}
\toprule
Tool & Evidence found by the inventory script & Expected & Reported & \\
\midrule
Claude Code & claude.exe running; VS Code extension anthropic.claude-code; global npm package @anthropic-ai/claude-code & active & active, high & \cmark \\
GitHub Copilot (IDE) & copilot-runtime.exe running in VS Code & active & active, high & \cmark \\
OpenAI Codex / ChatGPT app & MSIX package OpenAI.Codex installed; codex.exe and ChatGPT.exe running & active & active, high & \cmark \\
Claude Desktop (incl. Cowork) & MSIX package Claude installed (use within 30 days not independently verifiable) & installed & recent, high & \cmark \\
OpenCode & installed program OpenCode 1.18.3 & installed & installed, high & \cmark \\
Cursor & \textasciitilde{}/.cursor folder present; Cursor not installed & residue & residue, medium & \cmark \\
Ollama & \textasciitilde{}/.ollama folder present; Ollama not installed & residue & residue, medium & \cmark \\
Perplexity Comet (agentic browser) & empty \%LOCALAPPDATA\%\textbackslash{}Perplexity folder; Comet not installed & residue & residue, medium & \cmark \\
github-copilot-cli & Copilot CLI not installed; \textasciitilde{}/.copilot is used by the Copilot runtime of VS Code & absent & -- & \cmark \\
\bottomrule
\end{tabular}


==> eval/results/tex/tab-overhead-admin.tex <==
\begin{tabular}{@{}l r r@{}}
\toprule
Stage & Median (ms) & p95 (ms) \\
\midrule
Processes & 29.7 & 32.5 \\
TCP table & 1.9 & 4.0 \\
DNS cache & 30.9 & 33.1 \\
Traces & 4.2 & 6.6 \\
Inventory & 30.0 & 32.3 \\
Environment & 0.5 & 1.3 \\
Candidate inspection & 58.3 & 62.4 \\
Correlation & 35.8 & 37.1 \\
\midrule
Scan duration (elapsed) & 168 & 174 \\
CPU time (all threads) & 469 & 578 \\
\bottomrule
\end{tabular}


==> eval/results/tex/tab-signals-admin.tex <==
\begin{tabular}{@{}l l r >{\raggedright\arraybackslash}p{5.4cm}@{}}
\toprule
Evidence kind & Layer & Episodes & Which \\
\midrule
LLM endpoint & L3 network & 6 & A02, A03, A09, A10, A11, C03 \\
LLM + shell & L2 runtime & 10 & A01, A02, A03, A04, A05, A06, A07, A08, A09, A11 \\
base URL & L2/L5 configuration & 1 & A07 \\
local LLM port & L3 network & 1 & A08 \\
inference module & L2 runtime & 1 & C01 \\
MCP server & L2 runtime & 2 & A09, C02 \\
\bottomrule
\end{tabular}

